A Comprehensive Survey of Deep Learning in Remote Sensing: Theories, Tools and Challenges for the Community

In recent years, deep learning (DL), a re-branding of neural networks (NNs), has risen to the top in numerous areas, namely computer vision (CV), speech recognition, natural language processing, etc. Whereas remote sensing (RS) possesses a number of unique challenges, primarily related to sensors and applications, inevitably RS draws from many of the same theories as CV; e.g., statistics, fusion, and machine learning, to name a few. This means that the RS community should be aware of, if not at the leading edge of, of advancements like DL. Herein, we provide the most comprehensive survey of state-of-the-art RS DL research. We also review recent new developments in the DL field that can be used in DL for RS. Namely, we focus on theories, tools and challenges for the RS community. Specifically, we focus on unsolved challenges and opportunities as it relates to (i) inadequate data sets, (ii) human-understandable solutions for modelling physical phenomena, (iii) Big Data, (iv) non-traditional heterogeneous data sources, (v) DL architectures and learning algorithms for spectral, spatial and temporal data, (vi) transfer learning, (vii) an improved theoretical understanding of DL systems, (viii) high barriers to entry, and (ix) training and optimizing the DL.

==> FL_app_table.tex <==
%
% Table of Feature leaning papers in remote sensing
%

\begin{table}[ht]
\caption{FL paper subject areas in remote sensing.} 
\label{table:FL_papers}
\begin{center}       
\begin{tabular}{|l|l|l|l|}
\hline
\rule[-1ex]{0pt}{3.5ex}  \textbf{Area} & \textbf{References} & \textbf{Area} & \textbf{References} \\
\hline
\hline

\rule[-1ex]{0pt}{3.5ex}  
Active Learning &
\cite{Li2010Semisupervised, Li2011Hyperspectral, Zhang2016Multimetric} &
Automated target/object detection & 
\cite{firat2014representation, Geiss2016ObjectBased, Han2015Object, yu2015rotation} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Change detection &
\cite{ghosh2011fuzzy, liu2016difference} &
Competitive and transfer learning & 
\cite{Nogami1997Remote, Othman2015Deep} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Compressive sensing/sparse FL & 
\cite{li2011class, liang2016hyperspectral, Tao2015Unsupervised} &
Content-based retrieval & 
\cite{napoletano2016visual, zhou2015high} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Contextual feature learning & 
\cite{lazebnik2006beyond, li2014joint, Lin2015Learning, ma2015hyperspectral, popescu2012contextual, soh1999texture, zhang2006pixel, zhang2013tensor, zhao2016spectral, Zhou2016Learning, Zhou2012SelfSupervised} &
Dictionary learning & 
\cite{charles2011learning} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Dimensionality reduction & 
\cite{Bruce2002Dimensionality, Chang1999Joint, du2003band, du2011random, licciardi2009feature, mojaradi2009dimensionality, serpico2001new} &
Extreme learning & 
\cite{Huang2014SemiSupervised} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Feature extraction and selection & 
\cite{ali2001using, arzuaga2003unsupervised, benediktsson2003classification, Brumby1999investigation, camps2010remote, chanussot1999fuzzy, Fu2011Discriminant, Hu2015Unsupervised, huang2015sparse, huang2013svm, kumar2001best, Li2014Multiple, liao2013semisupervised, Mendenhall2008RelevanceBased, Mendenhall2006Generalized, Opitz2006Automated, PiedraFernandez2010Feature, roberts2013applications, romero2016unsupervised, Sermanet2013Pedestrian, singh2016learning, slavkovikj2016unsupervised, tsagkatakis2016deep, Tuia2015Multiclass, Tuia2014Automatic, wei2015latent, windrim2016unsupervised, yang2010nonparametric, yao2003genetic, yang2015learning, Yu2002Genetic, Zhang2015Automatic, Zhang2013Local, zhao2015combining, zou2015deep} &
Feature fusion & 
\cite{lisini2006feature, segl2003fusion, zhang2012combining, zhong2015scene} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Forestry model estimation & 
\cite{GarciaGutierrez2014Evolutionary, IzquierdoVerdiguier2014Semisupervised} &
HSI/MSI/SAR classification & 
\cite{alajlan2013using, castaings2010influence,  Chen2016Deep, DeDeuge2013Unsupervised, Gurram2014Coalition, Harvey2002Comparison, li2012spatial, meher2007wavelet, pierce1994knowledge, xie2014multilayer, zhao2016scene} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Image enhancement & 
\cite{yang2008fuzzy} &
Land Cover/Land Use Classification & 
\cite{bazi2009automatic, karalas2015deep, pacifici2009neural} \\
\hline
\rule[-1ex]{0pt}{3.5ex}  
Manifold/subspace/3D learning & 
\cite{campos2015shared, CamposTaberner2016Processing, jia2015laplacian, li2014nearest, Lin2008Riemannian, Ravannakhsh2017Deep, yu2015learning, zhou2015discriminative, zhu2015three} &
Multiple-kernel learning & 
\cite{gu2012representative, gu2016nonlinear, li2013generalized, menon2015hyperspectral, Subrahmanya2010Sparse, tuia2010learning} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Sampling analysis & 
\cite{hu2015comparative} &
Semantic annotation & 
\cite{lienou2010semantic, Dohan2015Learning, gleason2010semantic} \\
\hline

\rule[-1ex]{0pt}{3.5ex}  
Super-resolution & 
\cite{Arun2016Deep} &
Vehicle detection and tracking & 
\cite{she2004vehicle, wen2015efficient} \\
\hline

\end{tabular}
\end{center}
\end{table} 

